EntSUM: A Data Set for Entity-Centric Summarization

Controllable summarization aims to provide summaries that take into account user-specified aspects and preferences to better assist them with their information need, as opposed to the standard summarization setup which build a single generic summary of a document. We introduce a human-annotated data set EntSUM for controllable summarization with a focus on named entities as the aspects to control. We conduct an extensive quantitative analysis to motivate the task of entity-centric summarization and show that existing methods for controllable summarization fail to generate entity-centric summaries. We propose extensions to state-of-the-art summarization approaches that achieve substantially better results on our data set. Our analysis and results show the challenging nature of this task and of the proposed data set.

==> TO_DO.tex <==
Writing:

- Appendix: position distribution of summary sentences within sentences that contain the entity (to show summary sentences are not just lead3 containing entity)

- ROUGE between agnostic and entity-centric summary, to compute from slide 83: https://docs.google.com/presentation/d/159U98MwyUh2PFIR518iDhS-gyu2P5OrUOuWu_fAoTmc/edit#slide=id.ge7b577714c_1_14
Mayank: This is a manual computation right?

- ROUGE and BERTscore between the two summaries for the same (document, entity) pair.
Mayank: 
ROUGE 1/2/Lsum:  71.7 62.6 69.0
Average Summary Length (Words):  75.45905420991926
Average Summary Length (Chars):  411.34025374855827
Average Summary Length (Sents):  2.33679354094579
BERTScore F1=0.809499

Dataset Link: https://drive.google.com/file/d/1AXrPUpCKaExBfAv-RMtX6IeMJw7WATqr/view?usp=sharing 


Future experiments: 
- train on CNN vs NYT on the same size data or train on full CNN/DM
- plot distribution of predictions in terms of sentence position
- error analysis

To discuss:
- title of paper?
Mayank: EntSum: A Dataset for evaluating Entity-Centric Summarization
- name of data set?
Mayank: EntSum/EntCentSum
Mounica: EntSum

Chen-Tse comments:
- The "mostly extractive" in the introduction may cause some questions from the reviewers. Like how extractive it is or why not say it's abstractive.
- I guess another question might come up is the substring matching method for simple coref. What if an entity appears twice for a document (due to the imperfect coref). Not sure if you can say more about this. To me, it is fine.
- Line 160: add space between "titles" and the citation
- The number of annotators described between line 332 and 342 are somewhat mentioned in the previous sections, too. It's totally fine, just in case you want to save some space.

Mayank: Tried addressing Chen-Tse's comments
